Data-Driven Distributionally Robust Safety Verification Using Barrier Certificates and Conditional Mean Embeddings

Algorithmic verification of realistic systems to satisfy safety and other temporal requirements has suffered from poor scalability of the employed formal approaches. To design systems with rigorous guarantees, many approaches still rely on exact models of the underlying systems. Since this assumption can rarely be met in practice, models have to be inferred from measurement data or are bypassed completely. Whilst former usually requires the model structure to be known a-priori and immense amounts of data to be available, latter gives rise to a plethora of restrictive mathematical assumptions about the unknown dynamics. In a pursuit of developing scalable formal verification algorithms without shifting the problem to unrealistic assumptions, we employ the concept of barrier certificates, which can guarantee safety of the system, and learn the certificate directly from a compact set of system trajectories. We use conditional mean embeddings to embed data from the system into a reproducing kernel Hilbert space (RKHS) and construct an RKHS ambiguity set that can be inflated to robustify the result w.r.t. a set of plausible transition kernels. We show how to solve the resulting program efficiently using sum-of-squares optimization and a Gaussian process envelope. Our approach lifts the need for restrictive assumptions on the system dynamics and uncertainty, and suggests an improvement in the sample complexity of verifying the safety of a system on a tested case study compared to a state-of-the-art approach.

==> operatorBasedCME.tex <==
% Swapped operator-based CME for measure-theoretic CME
% Following is the prior operator-based CME text
For this, we introduce the concepts of Gram matrix and covariance operator.

%\medskip

%\noindent\textbf{Notation:}
Given a set $\hat X:=[\hat{x}_1,\ldots,\hat{x}_N]\T$ of i.i.d. samples $\hat{x}_i\in\X$, we define the \emph{Gram matrix} or \emph{Grammian} $K_{\hat{X}\hat{X}}$ of a kernel $k_x:\X\times\X\rightarrow\R$ as
$$K_{\hat{X}\hat{X}}:=k_x(\hat{X},\hat{X})=\begin{bmatrix}
	k_x(\hat{x}_1,\hat{x}_1) & \ldots & k_x(\hat{x}_1,\hat{x}_N)\\ \vdots & \ddots & \vdots\\ k_x(\hat{x}_N,\hat{x}_1) & \ldots & k_x(\hat{x}_N,\hat{x}_N)
\end{bmatrix}.$$
Furthermore, we define the vector-valued function $$k_{x\hat{X}}(x)  := k_x(x,\hat{X}) = [k_x(x,\hat{x}_1),\ldots,k_x(x,\hat{x}_N)].$$
%For the implicit embedding $\phi_x(\cdotx)$ of an RKHS $\Hilbert_{k_x}$ we have $k_x(x,x')=\phi_x(x)\T\phi_x(x')$.
As a generalization of the covariance matrix, the \emph{cross-covariance operator} $C_{xy}:\Hilbert_{k_x}\rightarrow\Hilbert_{k_y}$ 
for random variables $(x,y)\sim P_{xy}\in\mathcal{P}(\X\times\Y)$
%introduced in \cite{Baker1973CrossCov} 
is given by the expression
$$C_{xy}:=\E_{xy\sim P_{xy}}[\phi_x(x)\otimes\phi_y(y)] -\mu_{k_x}(P_x)\otimes\mu_y(P_y),$$
with 
$k_y:\Y\times\Y\rightarrow\R$ the characteristic kernel of the RKHS $\Hilbert_{k_y}$, $\phi_y:\Y\rightarrow\Hilbert_{k_y}$ its canonical embedding, 
marginal probability distributions $P_x\in\mathcal{P}(\X)$, $P_y\in\mathcal{P}(\Y)$,
% $P_{xy}\in\mathcal{P}(\X\times\Y)$,
and $\otimes$ the tensor product \cite{Baker1973CrossCov}. The \emph{covariance operator} $C_{xx}$ is recovered for \red{$x=y$}. \Oliver{Technically I want to say that instead of considering to different random variables $X,Y$ I am now looking at $Y=X$.}

\medskip





%The following definition is a generalization of the covariance matrix, originally introduced in \cite{Baker1973CrossCov}.
%\begin{definition}[Cross-covariance operator]
%	The \emph{cross-covariance operator} $C_{xy}:\Hilbert_{k_x}\rightarrow\Hilbert_{k_y}$ is defined as 
%	$$C_{xy}:=\E_{xy}[\phi_x(x)\otimes\phi_y(y)] -\mu_{k_x}(x)\otimes\mu_y(y),$$
%	where $\otimes$ is the tensor product.
%\end{definition}
With the following definition, we embed conditional probability distributions into Hilbert space \cite{Song2009CondEmbed}.
\begin{definition}[Conditional mean embedding]\label{def:condMeanEmbed}
	Given two RKHSs $(\Hilbert_{k_x},\Hilbert_{k_y})$ with characteristic kernels $k_x:\X\times\X\rightarrow\R$ and $k_y:\Y\times\Y\rightarrow\R$,
	the \emph{conditional mean embedding} of a conditional probability distribution $P:\X\times\borel{\Y}\rightarrow[0,1]$
	satisfying $\E_{y\sim P(\cdotx|x)}[\bar\phi_y(y)|x]\in\Hilbert_{k_y}$, $\forall x\in\X$ for all functions $\bar\phi_y:\Y\rightarrow\Hilbert_{k_y}$ 
	%	\pdfmargincomment{This is especially critical for continuous domains.}
	is a mapping $\mu_{y|x}:\X\times\mathcal{P}(\Y)\rightarrow\Hilbert_{k_y}$ s.t.
	\begin{equation*}
		\mu_{y|x}(P)(x) := \E_{y|x}[\phi_y(P(y|x))|x] = C_{yx}C_{xx}^{-1}\phi_x(x).
	\end{equation*}
	
\end{definition}
Analogous to the non-conditional case, we can compute the expected value of a function $f\in\Hilbert_{k_y}$
%\pdfmargincomment{Can we formulate this as a mapping from a space to another?} 
via its inner product with the conditional mean embedding, i.e.,
\begin{equation}
	\E_{y|x}[f(P(y|x))|x] = \innerH{f}{{\mu}_{y|x}(P)(x)}{\Hilbert_{k_y}}.\label{eq:innerProdCond}
\end{equation}
Since in some cases the conditional mean embedding might be unknown and shall be estimated from data, we extend Prop.~\ref{prop:empMeanEmbed} to conditional distributions \cite{Song2009CondEmbed}.
\begin{proposition}[Empirical (conditional) mean embedding]\label{prop:empCondMeanEmbed}
	Let a finite set $(\hat{X},\hat{Y}):= \{(\hat{x}_1,\hat{y}_1),\ldots,(\hat{x}_N,\hat{y}_N)\}$ of i.i.d. samples $\hat{y}_i\sim P(\cdotx|\hat{x}_i)$
	from a conditional probability distribution $P:\X\times\borel{\Y}\rightarrow[0,1]$ be given.
	For two kernels $k_x:\X\times\X\rightarrow\R$ and $k_y:\Y\times\Y\rightarrow\R$
	the \emph{empirical (conditional) mean embedding} of $P$ given $(\hat{X},\hat{Y})$ is
	a mapping $\hat{\mu}_{y|x}^N:\X\times\mathcal{P}(\Y)\rightarrow\Hilbert_{k_y}$ given by
	\begin{equation*}
		\hat{\mu}_{y|x}^N(x) := k_{x\hat{X}}(x)\left[ K_{\hat{X}\hat{X}}+N\lambda I_N\right]^{-1} \phi_y(\hat{Y}),
	\end{equation*}
	%	where $w(x) := k_{x}(x)\T(K_{x}+N\lambda I_N)^{-1}\in\R^N$ 
	%	with the Gram matrix $K_{x}$ 
	%	and row vector $k_{x}(x)\T := [k_x(\hat{x}_1,x),\ldots,k_x(\hat{x}_N,x)]$ 
	with 
	%	$\phi_{\hat{Y}}:=\phi_y(\hat{Y})$ and 
	a regularization constant $\lambda\geq0$.
\end{proposition}
Note that we adopt a notation similar to Gaussian process (GP) regression (cf. \cite{Kanagawa2018GPvsKernel}) and omit the dependence of $\hat{\mu}_{y|x}^N$ on $P$ for ease of use. 
Here and in the following, we will assume $[K_{\hat{X}\hat{X}}+N\lambda I_N]$ (or equivalent terms) to be invertible. \Oliver{Don't require this if the regularization constant is strictly positive.}
Then, by virtue of the reproducing property we have for any function $f\in\Hilbert_{k_y}$: $$\innerH{f}{\hat{\mu}^N_{y|x}(x)}{\Hilbert_{k_y}} = k_{x\hat{X}}(x)\left[ K_{\hat{X}\hat{X}}+N\lambda I_N\right]^{-1} f(\hat{Y}).$$
% where $f_{\hat{Y}}:=f(\hat{Y})$.
Note that the results in Prop.~\ref{prop:concentrationBounds} can also be applied to relate conditional mean embeddings (Def.~\ref{def:condMeanEmbed}) and their empirical counterparts from Prop.~\ref{prop:empCondMeanEmbed}

% \section{Main Result}
%\gray{We define an ambiguity set based on the maximum mean discrepancy (MMD) of two conditional distributions as follows.
	%\begin{definition}[MMD ambiguity set]
	%	Let $\hat{\mu}^N_{x|y}$ be the empirical mean embedding of $P:\X\times\borel{\Y}\rightarrow\R_{\ge 0}$ based on a finite data set $\data_{y|x}$. Then, the \emph{MMD ambiguity set} with radius $\varepsilon\geq 0$ is given by
	%	$$\amb := \left\lbrace  P\in\mathcal{P}(\X\times\borel{\Y}) \,\big|\, ||\mu_{x|y}(P)-\hat{\mu}^N_{x|y}||_{\Hilbert_{k_x}} \leq \varepsilon\right\rbrace.$$
	%\end{definition}}
	%The following \red{sharp} finite sample guarantees for i.i.d. samples is taken from the paper \cite{Nemmour2022FiniteSampleGuarantee}.
	%\begin{theorem}[Finite sample guarantees]\label{prop:concentrationBounds}
	%	Let $N$ i.i.d. samples from the population distribution $P^\star\in\mathcal{P}(\X\times\borel{\Y})$ be given, i.e., $(\hat{x}_1,\hat{y}_1),\ldots,(\hat{x}_N,\hat{y}_N)$ with $\hat{y}_i\sim P^\star(\hat{x}_i)$. 
	%	Furthermore, let $k_y:\Y\times\Y\rightarrow\R$ be the characteristic kernel of the RKHS $\Hilbert_{k_y}$.
	%	Then, it holds for the empirical conditional mean embedding $\hat{\mu}^N_{y|x}$ that with confidence level $\delta\in(0,1)$ we have
	%	\begin{equation*}
		%		\P\left\lbrace  ||\mu_{y|x}(P^\star)-\hat{\mu}^N_{y|x}||_{\Hilbert_{k_y}} \leq \varepsilon \right\rbrace \geq 1-\delta,
		%	\end{equation*}
	%	with radius $\varepsilon := \sqrt{\frac{C}{N}} + \sqrt{\frac{2C\log(1/\delta)}{N}}$ and a constant $C\leq\infty$ such that $\sup_{y\in\Y} k_y(y,y)\leq C$.
	%\end{theorem}
	%Note that the concentration bounds provided by Thm.~\ref{prop:concentrationBounds} are usually overly conservative and can be improved using a MMD bootstrap theme as in \cite{Nemmour2022FiniteSampleGuarantee}.
